MLComp: A Methodology for Machine Learning-based Performance Estimation and Adaptive Selection of Pareto-Optimal Compiler Optimization Sequences

Embedded systems have proliferated in various consumer and industrial applications with the evolution of Cyber-Physical Systems and the Internet of Things. These systems are subjected to stringent constraints so that embedded software must be optimized for multiple objectives simultaneously, namely reduced energy consumption, execution time, and code size. Compilers offer optimization phases to improve these metrics. However, proper selection and ordering of them depends on multiple factors and typically requires expert knowledge. State-of-the-art optimizers facilitate different platforms and applications case by case, and they are limited by optimizing one metric at a time, as well as requiring a time-consuming adaptation for different targets through dynamic profiling. To address these problems, we propose the novel MLComp methodology, in which optimization phases are sequenced by a Reinforcement Learning-based policy. Training of the policy is supported by Machine Learning-based analytical models for quick performance estimation, thereby drastically reducing the time spent for dynamic profiling. In our framework, different Machine Learning models are automatically tested to choose the best-fitting one. The trained Performance Estimator model is leveraged to efficiently devise Reinforcement Learning-based multi-objective policies for creating quasi-optimal phase sequences. Compared to state-of-the-art estimation models, our Performance Estimator model achieves lower relative error (<2%) with up to 50x faster training time over multiple platforms and application domains. Our Phase Selection Policy improves execution time and energy consumption of a given code by up to 12% and 6%, respectively. The Performance Estimator and the Phase Selection Policy can be trained efficiently for any target platform and application domain.

==> COGUTS - DATE2021 (Copy)3/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%						Acronyms							   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[acronym]{glossaries} % Acronyms


% \newacronym{<acr>}{<abbr>}{<full>}

\newacronym{pe}{PE}{Performance Estimator}
\newacronym{pss}{PSS}{Phase Sequence Selector}

\newacronym{iot}{IoT}{Internet of Things}
\newacronym{cps}{CPS}{Cyber-Physical System}
\newacronym{ml}{ML}{Machine Learning}
\newacronym{sl}{SL}{Supervised Learning}
\newacronym{rl}{RL}{Reinforcement Learning}

\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{mle}{MLE}{Maximum Likelihood Estimation}
\newacronym{ir}{IR}{Intermediate Representation}

==> COGUTS - DATE2021 (Copy)3/sections/0_abstract.tex <==
% currently at 233 words
Embedded systems have proliferated in various consumer and industrial applications with the evolution of Cyber-Physical Systems and the Internet of Things.
These systems are subjected to stringent constraints so that embedded software must be optimized for multiple objectives simultaneously, namely reduced energy consumption, execution time, and code size.
Compilers offer optimization phases to improve these metrics. However, proper selection and ordering of them depends on multiple factors and typically requires expert knowledge.
% Standard optimizers select and order optimization phases according to heuristics that are not tailored to the different target platforms and application domains.
State-of-the-art optimizers facilitate different platforms and applications case by case, and they are limited by optimizing one metric at a time, as well as requiring a time-consuming adaptation for different targets through dynamic profiling.
% Therefore, it is an extremely time-consuming process.

To address these problems, we propose the novel \textit{MLComp} methodology, in which optimization phases are sequenced by a Reinforcement Learning-based policy. Training of the policy is supported by Machine Learning-based analytical models for quick performance estimation, thereby drastically reducing the time spent for dynamic profiling.
%We train our Performance Estimator model using results from profiling on a given target platform.
In our framework, different Machine Learning models are \textit{automatically} tested to choose the best-fitting one.
The trained Performance Estimator model is leveraged to efficiently devise Reinforcement Learning-based multi-objective policies for creating quasi-optimal phase sequences.

Compared to state-of-the-art estimation models, our Performance Estimator model achieves lower relative error ({$<\mathrm{\textbf{2\%}}$}) with up to 50$\times$ faster training time over multiple platforms and application domains. Our Phase Selection Policy improves execution time and energy consumption of a given code by up to 12\% and 6\%, respectively.
%While the models are trained for a given target platform and set of applications, our methodology is general, so that the performance estimator model and the phase selection policy can be trained efficiently for any target platform and application domain.
The Performance Estimator and the Phase Selection Policy can be trained efficiently for any target platform and application domain.

\vspace*{-2mm}


==> COGUTS - DATE2021 (Copy)3/sections/1_introduction.tex <==
%\vmR{Big framework/system image with inputs and outputs, light blue for novel contributions}

%\subsection{Introduction and Target Research Problem}
%\david{I removed subsectioning from Introduction.}



%Field and use-cases:
%\begin{itemize}
%    \item IoT, minimization of power, code size and execution time for constrained-envelope embedded systems
%\end{itemize}

% Professor Shafique suggested to have:
% - 2-3 lines about the topic (IoT, compilers)
% - 2-3 lines about the main problem (efficiency in obtaining optimal optimizations)
% - categorized sota (to use them as basis of the motivational case study later), in comparison with our approach and our results.

% Then a subsection with the motivational case study.

% A subsection with scientific challenges to overcome.

% A list of novel contributions addressing specific challenges.

% Finally, a subsection with a quick overview of evaluation and results, and the main message from the paper.

%Intro:
%\begin{itemize}
%    \item number and complexity of embedded systems are constantly growing~\cite{Atzori2010,Samie2016}
%    \item advent of \gls*{iot} and \glspl*{cps}, and their subsequent applications such as autonomous driving~\cite{Liu2017}, automated manufacturing plants~\cite{Yaqoob2014}, and mobile health monitoring systems~\cite{Massot2009}
%    \item these systems are extremely resource-constrained, requiring latency-limited real-time operation with very low power budget
%    \item software running on them must be exceptionally optimized and tailored to the specific hardware
%\end{itemize}

The number and complexity of embedded systems are constantly growing~\cite{Atzori2010,Samie2016}.
Recent years saw an advent of the \gls*{iot} and \glspl*{cps}, and their subsequent applications~\cite{Liu2017,Yaqoob2014,Massot2009}.
These systems are tightly resource-constrained, requiring latency-limited real-time operation with a very low power budget.
Software running on them must be optimized and tailored to the specific hardware.

%Problem:
%\begin{itemize}
%    \item major optimizing compilers (e.g., LLVM~\cite{Lattner2004} and GCC~\cite{Stallman2020}) provide an ever-increasing number of optimization phases to improve operational characteristics of embedded software
%    \item optimal selection and ordering of the optimization phases depend on the program to be compiled and its target platform, as well as the final optimization objective
%    \item value of the objective function must be estimated at compile-time to tune the selection and ordering processes
%\end{itemize}

Major optimizing compilers, like LLVM~\cite{Lattner2004} and GCC~\cite{Stallman2020}, provide an ever-increasing number of optimization phases to improve operational characteristics of embedded software.
The phases are applied during compilation in sequence.
Their optimal selection and ordering depend on the program to be compiled and on the target platform, as well as on the final optimization objective.
The value of the objective function must be estimated at compile-time to tune phase sequencing.

%State of the art:
%\begin{itemize}
%    \item standard phase selection and ordering policies in optimizing compilers~\cite{Lattner2004, Stallman2020} are fixed algorithms that have been tuned for the average case
%    \item state-of-the-art approaches for choosing the optimization phases are based on \gls*{ml}~\cite{Ashouri2017, Fursin2011, Kulkarni2012, ashouriSurveyCompilerAutotuning2018} and other adaptive mechanisms~\cite{Blackmore2017, Pallister2015}
%    \item some approaches are dealing with phase selection only~\cite{Ashouri2016,Fursin2011} and ignore ordering, which would be important for the quality of generated code~\cite{Almagor2004}
%    \item most works optimize for a specific characteristic, like execution time~\cite{Blackmore2017,Ashouri2016,Ashouri2017,Kulkarni2012} or energy consumption~\cite{Pallister2015}
%    \item state of the art is not generic, it provides optimal results only in a limited environment and for specific objectives
%    \item they implement profiling to gather the required characteristics and objectives, which is time expensive as it requires direct execution
%    \item we require a fast-yet-accurate estimation method to reduce the total training time
%    \item state-of-the-art models can be distinguished as \gls*{ml}-based~\cite{diopPowerModelingHeterogeneous2014,balaprakashAutoMOMMLAutomaticMultiobjective2016,liAccurateEfficientProcessor2009} and formal~\cite{bonaEnergyEstimationOptimization2002,vandensteenAnalyticalProcessorPerformance2016,laurentFunctionalLevelPower2004} models
%    \item \gls*{ml}-based models tend to use more accurate sensors and interfaces to estimate the power, which requires external modifications, and focus on a single characteristic, obtaining good results by employing a small selection of models (at most 10-15\% relative error)
%    \item formal models estimate the power using formulas and accurate simulations of switching activity, but this requires more knowledge on the internal workings of the target platform, while guaranteeing very high accuracy
%\end{itemize}

Standard phase selection and ordering policies in optimizing compilers~\cite{Lattner2004, Stallman2020} are fixed algorithms that have been tuned for the average case and do not exactly fit to actual use-cases.
State-of-the-art approaches for choosing the optimization phases are based on \gls*{ml}, e.g. \gls*{sl} and \gls*{rl}~\cite{Ashouri2017, Fursin2011, Kulkarni2012, ashouriSurveyCompilerAutotuning2018}, and other adaptive mechanisms~\cite{Blackmore2017, Pallister2015}.
Some approaches ignore phase ordering and deal with phase selection only~\cite{Fursin2011,Ashouri2016}, while the order is important for the quality of the generated code~\cite{Almagor2004}.
Most of the works optimize programs for one specific metric only, like execution time~\cite{Ashouri2017,Kulkarni2012,Blackmore2017,Ashouri2016} or energy consumption~\cite{Pallister2015}.
\textit{The state-of-the-art solutions are typically not generic, i.e.,  they provide good results only in a limited environment and for one specific metric at a time.}
Moreover, these methods gather the required metrics by profiling execution, which is super-expensive in time, and should be replaced by a fast-yet-accurate estimation method to reduce the total adaptation time.

State-of-the-art estimation models can be distinguished as \gls*{ml}-based~\cite{diopPowerModelingHeterogeneous2014,balaprakashAutoMOMMLAutomaticMultiobjective2016,liAccurateEfficientProcessor2009} and formal~\cite{bonaEnergyEstimationOptimization2002,vandensteenAnalyticalProcessorPerformance2016,laurentFunctionalLevelPower2004} ones.
\gls*{ml}-based models tend to use accurate sensors and interfaces to estimate the power, and hence require external modifications. However, these methods focus only on a single metric and employ only a small selection of models with at most 5\% relative error.
Formal models estimate the power using formulas and accurate simulation of switching activity that guarantees high accuracy. However, they require deep knowledge of the internal details of the target platform.


%\subsection{Motivation}

% \begin{figure}[t]
%     \centering
%     \includesvg[width=0.8\linewidth]{images/motivation.svg}
%     \caption{}
%     \label{fig:motivation}
% \end{figure}

\begin{table}[]
\caption{
Comparison of
\gls*{ml}-based state-of-the-art
phase selection policies.}
\vspace*{-1mm}
\resizebox{\linewidth}{!}{%
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
                                                                                           &                                                       & \multicolumn{3}{c|}{\textbf{Metrics}}                                                                                                                             &                                                                                     &                                                                                       \\ \cline{3-5}
\multirow{-2}{*}{\textbf{Solution}}                                                        & \multirow{-2}{*}{\textbf{Technique}}                  & \textit{\begin{tabular}[c]{@{}c@{}}Execution\\ Time\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Energy\\ Consumption\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Code\\ Size\end{tabular}}       & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Phase\\ Ordering\end{tabular}}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Dynamic\\ Features\end{tabular}}} \\ \hline
COBAYN \cite{Ashouri2016,Ashouri2014}                                     & \acrshort*{sl}                        & X                                            &                                                  &                                         & No                                        & Profiling                                   \\ \hline
Milepost GCC \cite{Fursin2011}                                            & \acrshort*{sl}                        & X                                            &                                                  & X                                       & No                                        & Profiling                                   \\ \hline
MiCOMP \cite{Ashouri2017}                                                 & \acrshort*{sl}                        & X                                            &                                                  &                                         & Static                                    & Profiling                                   \\ \hline
\cite{Kulkarni2012}                                                       & \acrshort*{rl}                        & X                                            &                                                  &                                         & Dynamic                                   & Profiling                                   \\ \hline
\cite{Ashouri2016a}                                                       & \acrshort*{sl}                        & X                                            &                                                  &                                         & Dynamic                                   & Profiling                                   \\ \hline
{\color[HTML]{FF0000} \textit{\textbf{MLComp (\acrshort*{pss})}}} & {\color[HTML]{FF0000} \textit{\textbf{\acrshort*{rl}}}} & {\color[HTML]{FF0000} \textit{\textbf{X}}}                     & {\color[HTML]{FF0000} \textit{\textbf{X}}}                         & {\color[HTML]{FF0000} \textit{\textbf{X}}}                & {\color[HTML]{FF0000} \textit{\textbf{Dynamic}}}            & {\color[HTML]{FF0000} \textit{\textbf{Prediction}}}           \\ \hline
\end{tabular}
}
\label{tab:pss}
\vspace*{-3.2mm}
\end{table}



\begin{table}[]
\caption{
Comparison of state-of-the-art performance estimators.}
\vspace*{-1mm}
\resizebox{\linewidth}{!}{%
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
                                                   &                                            &                                                                                       & \multicolumn{4}{c|}{\textbf{Metrics}}                                                                                                                                                                                                                                                   &    &                                                                        \\ \cline{4-7}
\multirow{-2}{*}{\textbf{Solution}}                & \multirow{-2}{*}{\textbf{Automation}}      & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Machine\\ Learning\end{tabular}}} & \textit{\begin{tabular}[c]{@{}c@{}}Execution\\ Time\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Energy\\ Consumption\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}\# Executed\\ Instructions\end{tabular}} & \textit{\begin{tabular}[c]{@{}c@{}}Average\\ Power\end{tabular}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Gathering\end{tabular}}} & \multirow{-2}{*}{\textbf{Accuracy}} \\ \hline
\cite{diopPowerModelingHeterogeneous2014}                                               & Limited                                           & Basic                                                                                     &                                                                   &                                                                       &                                                                             & X                                                                & Profiling   & $\thicksim$5\%                                                               \\ \hline
\cite{balaprakashAutoMOMMLAutomaticMultiobjective2016}                                        & Limited                                          & Basic                                                                                     & X                                                                 &                                                                       &                                                                             & X                                                                & Profiling & $\thicksim$5\%                                                                 \\ \hline
\cite{liAccurateEfficientProcessor2009}                                                 & Limited                                           & Basic                                                                                     &                                                                   &                                                                       &                                                                             & X                                                                & Simulation   & $\thicksim$3\%                                                              \\ \hline
\cite{bonaEnergyEstimationOptimization2002}                                               & No                                           &  No                                                                                     &                                                                   &                                                                       &                                                                             & X                                                                & Simulation  & $\thicksim$2\%                                                               \\ \hline
\cite{vandensteenAnalyticalProcessorPerformance2016}                                        & Limited                                           & No                                                                                      & X                                                                 &                                                                       &                                                                             & X                                                                & Profiling & $\thicksim$7\%                                                                 \\ \hline
\cite{laurentFunctionalLevelPower2004}                                            & No                                           & No                                                                                      &                                                                   &                                                                       &                                                                             & X                                                                & Simulation &  $<$5\%                                                              \\ \hline
{\color[HTML]{FF0000} \textit{\textbf{\begin{tabular}[c]{@{}c@{}}MLComp\\(\acrshort*{pe})\end{tabular}}}} & {\color[HTML]{FF0000} \textit{\textbf{Full}}} & {\color[HTML]{FF0000} \textit{\textbf{Advanced}}}                                            & {\color[HTML]{FF0000} \textit{\textbf{X}}}                        & {\color[HTML]{FF0000} \textit{\textbf{X}}}                            & {\color[HTML]{FF0000} \textit{\textbf{X}}}                                  & {\color[HTML]{FF0000} \textit{\textbf{X}}}                       & {\color[HTML]{FF0000} \textit{\textbf{Profiling}}} &  {\color[HTML]{FF0000} \textit{\textbf{$<$2\%}}}                      \\ \hline
\end{tabular}%
}
\label{tab:pe}
\vspace*{-5mm}
\end{table}

%\begin{itemize}
%    \item power modeling: most of the works focus on hand-tuned high-level models, few works use machine learning algorithms. They select a single algorithm to be used for the dataset, neglecting the possibility that different models may adapt better to different application-platform sets; thus, long human-made analysis and design are still required;
%    \item phase sequence selector: many works have used machine learning for obtaining optimal phase sequences \cite{ashouriSurveyCompilerAutotuning2018}, but the focus neglects \gls{rl} policies and alternative objectives;
%    \begin{itemize}
%        \item they optimize for one objective, so they cannot meet a Pareto-optimal distribution of relevant objectives;
%        \item they train on data obtained by profiling, which might require custom hardware and software components as well as have long execution time;
%    \end{itemize}
%\end{itemize}

Our work aims at overcoming specific limitations of state-of-the-art solutions in compiler phase sequencing and performance estimation. Tables~\ref{tab:pss} and~\ref{tab:pe} highlight the shortcomings of major state-of-the-art with respect to different properties/features, and show comprehensive and superior coverage of our \textit{MLComp} methodology.
Our phase sequence selector possesses the following key attributes:
\begin{itemize}[leftmargin=*]
    \item It utilizes \textit{\gls*{rl}}, which has been given little attention in the literature for obtaining optimal phase sequences.
    \item It optimizes programs for multiple objectives in contrast to typical single-objective optimizations.
    \item It supports fast adaptation for different application domains.
\end{itemize}
The latter is enabled by fast performance estimation in the adaptation phase, which requires proper performance modeling of target platforms. To adapt to the different target platforms efficiently, potential models need to be evaluated and the best-fitting one selected. This process, which is usually done by manual analysis and design~\cite{laurentFunctionalLevelPower2004}, is automated in our solution.

%List of open challenges, not addressed by SOTA:
%\begin{itemize}
%    \item analysis and trade-offs of different machine learning models for power modeling, not addressed by state-of-the-art as most models are specific to a certain configuration, thus they do not require adapting to different application-platform sets;
%    \item adaptive policies for phase sequence selection, as different application-platform sets may have different optimal choices for Pareto-optimal results;
%\end{itemize}

Our efforts are focused on the following \textit{scientific challenges}, which, to the best of our knowledge, have not been addressed in the literature before:
\begin{itemize}[leftmargin=*]
    \item automatic evaluation of different \gls*{ml}-based performance models to support adaptation to different platforms;
    \item efficient training of adaptive phase sequence selection policies for multi-objective optimization of programs.
\end{itemize}


%Main target research problem, why it is worthy to investigate:
%\begin{itemize}
%    \item develop a fast and efficient way of estimating power and dynamic features given a set of chosen applications and platforms, to adapt to the different characteristics, while providing results targeted to the chosen set. Such models can be implemented to analyze different domain-specific applications and their specific hardware, allowing faster and accurate modeling over standard estimation methods;
%    \item implement adapting ML-based policies for phase sequence selection. This will allow faster time-to-market with improved performance, reducing the designer effort while guaranteeing enough flexibility for usage in different scenarios and applications;
%\end{itemize}





%\davidi{Here should come a short paragraph summary of Motivation to support the flow. Details in the following section.}

% \blue{Few works in literature use \gls{ml} algorithms for power modeling~\cite{diopPowerModelingHeterogeneous2014,bonaEnergyEstimationOptimization2002}. They select a single algorithm for certain conditions. Our \gls{pe} can be adapted by analyzing trade-offs among different \gls{ml} models.}\david{@Alessio: Please check this too.}
% Phase selection and phase ordering are in a similar situation: there are \gls{ml}-based approaches~\cite{ashouriSurveyCompilerAutotuning2018} with models selected for certain conditions. Our \gls{pss} leverages \gls{rl} to adapt the policy for different applications and platforms.



%\subsection{Novel Contributions \& Key Results}





%\subsection{Main Scientific Results}

\textbf{Novel Contributions:} To address the above challenges, we propose a novel methodology \textit{MLComp} that employs:
\begin{itemize}[leftmargin=*]
    \item \textbf{adaptive analytical models} for estimating energy consumption and execution time, which are trained on %static and dynamic
    features of target applications executing on a given target platform; and
    \item \textbf{adaptive phase sequence selection policies}, which can be trained for quasi-Pareto-optimal code size, energy consumption, and execution time of target applications running on a target platform.
\end{itemize}

The paper makes the following additional \emph{novel contributions}:
\begin{itemize}[leftmargin=*]
    \item \textbf{testing environment} to collect static and dynamic features of target applications on a target platform;
    \item \textbf{framework to adapt performance models} by analyzing and modeling energy consumption and execution time based on the collected code features; and
    \item \textbf{training framework} for \gls*{rl}-based adaptation of phase selection policies with respect to estimated dynamic features, and utilizing trained policies in LLVM.
\end{itemize}

After presenting a brief overview of the required background knowledge in Section \ref{sec:background}, we explain our novel \textit{MLComp} methodology in Section \ref{sec:methodology}. Experimental setup is explained in Section \ref{sec:experimental_setup}, which is followed by our results in Section \ref{sec:evaluation}. Conclusion is drawn in Section \ref{sec:conclusion}.




% \blue{\textbf{Suggested Chain of Arguments:} If you answer the following questions, this will form a connected chain of argument. Note, for each statement/claim that you provide, you should provide concrete numbers, solid references, and/or your own analysis to support them properly. Every claim related to the contributions should be corroborated by proper in-depth results and technical discussion.
% %
% \begin{itemize}
% \item What is the main area and relevant problem that you are going to target in this paper? Why is this problem relevant and important for the research community?
% %
% \item What are most important state-of-the-art in this area that also aim at the similar problem? Give brief description in categorized form. Detailed related work should be put together in a separate section.
% %
% \item What are the main limitations of the above state-of-the-art techniques? Considering this, formulate the concrete research problem that you will target in this paper, and discuss associated scientific challenges which have to be addressed to meet that goal.
% %
% \item What are your key novel contributions and what makes them novel? Give concrete description that can give a glimpse of the new technique, methodology, etc.
% %
% \item What are the most important results? Give glimpse about the realistic experimental setup, so that results are credible. Also provide a  link, if you are going to  make the tool chain and results open-source.
% %
% \item Paper Organization: Afterwards, provide a concise paper organization stating what would come under different sections. 
% %
% \end{itemize}
% }

% \blue{\textbf{Target Problem and Associated Scientific Challenges:}
% Put the concerte research problem targeted in this paper here followed by a list of the associated scientific challenges. These challenges are then directly addressed by different novel contribution stated below.
% \begin{itemize}
% \item TODO
% \item TODO
% \item TODO
% \end{itemize}
% }

% \textbf{Main Contributions:}
% \begin{itemize}
%     \item An ML-based optimization method that improves optimizing compilers by applying standard optimization passes in custom sequences that are adapted for the individual programs.
%     \item Implementation of the method as (1) a custom LLVM optimization pass that uses a pre-trained PyTorch model via libtorch and (2) a training bench in Python that allows training/refining/retargeting the PyTorch model for different platforms and/or application domains.
%     \item Evaluating the proposed method and implementation with the RISC-V BEEBS benchmarks.
% \end{itemize}

% \blue{\textbf{TODO for David:} Make  figure connecting different novel contributions and guiding to their respective sections. Input and Outputs should be clearly mentioned.}

% \blue{\textbf{Paper Organization:}
% The rest of the paper is organized as follows. Section II presents the related work in XYZ and XYZ areas. Section III provides the necessary background knowledge to understand the contributions of this paper. Section IV provides an overview of our methodology followed by details of different contributions. Section V presents the results and discussion, followed by the conclusion in Section VI.}

==> COGUTS - DATE2021 (Copy)3/sections/2_background.tex <==
\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/compiler_flow.svg}
    \caption{A compiler converts source code into an executable by passing it through optimizations in \acrlong*{ir}.}
    \label{fig:compiler_flow}
    \vspace*{-6mm}
\end{figure}



%Compilers:
%\begin{itemize}
%    \item A compiler turns high-level software source into machine executable code.
%    \item A compiler consists of 3 main parts: a \emph{front end} that transforms source code into \gls{ir} form, a \emph{middle end} that performs analyses and transformations in \gls{ir}, and a \emph{back end} that turns \gls{ir} into target-specific executable.
%    \item Optimizing transformations can be performed in each part. Front end optimizations are specific for a programming language. Back end optimizations are low-level transformations to tune for the hardware architecture. Middle end optimizations are general and independent from the source language and the target architecture. However, they effect the performance differently depending on the target.
%    \item FIGURE with compiler flow, highlighting the part on which we focus on, we focus on middle end optimizations to be general
%\end{itemize}

A compiler converts a given software code implemented in a high-level programming language into machine executable code.
The compilation flow is divided into 3 main parts:
\begin{enumerate}[leftmargin=*]
    \item the \emph{front end} transforms source code into the compiler's \gls*{ir};
    \item the \emph{middle end} performs analyses and transformations in \gls*{ir} to ensure quality and prepares for code generation;
    \item the \emph{back end} generates a target-specific executable from \gls*{ir}.
\end{enumerate}
Optimizing transformations are performed in each stage. Optimizations in the front end are specific to the programming language, while those in the back end tune hardware-specific low-level details. We work with \gls*{ir}-level optimizations in the middle end as depicted in Fig.~\ref{fig:compiler_flow}. Those optimizations are general and applied independently to the source language and target platform. However, they can affect the performance in different ways depending on the target, which calls for their adaptive selection and ordering.


%Machine Learning and Reinforcement Learning:
%\begin{itemize}
%    \item machine learning is used to learn a model representation that can fit input data to output predictions;
%    \item at each pass, the model predicts the outputs given the input data, and the results are used to update the model weights to return predictions closer to the correct ones;
%    \item reinforcement learning, on the other hand, uses a reward-based system to learn the operations which should be done from the current status of the system itself;
%\end{itemize}

Standard \gls*{ml} methods are available to solve different kinds of algorithmic and modeling problems.
\gls*{sl}~\cite{Simeone2017} is used to learn a model representation that can fit input data to output predictions.
The model is trained in iterative passes. In each pass, the model predicts output for the given input data, and the results are used to update the model weights to return predictions closer to the correct ones.
\gls*{rl}~\cite{Francois-lavet2018}, on the other hand, uses a reward-based system to learn the operations which should be done from the current state of the system itself. The reward reflects how an operation contributes to reaching the objective.

%\subsection{Program Characterization}

%\begin{itemize}
%    \item \gls{ml} techniques need features that capture important characteristics of programs
%    \item Possible features: source code features including application code in a programming language and the compiler intermediate representation, graph-based features with explicit data and control dependencies, as well as architecture dependent and independent dynamic features
%    \item however, programming language source features are language-dependent, and dynamic features are expensive to obtain for each sample.
%\end{itemize}

Programs are represented by their characterising features for \gls*{ml} approaches.
The main types of program features are:
\begin{itemize}[leftmargin=*]
    \item \emph{source code features} that characterize application code in a programming language and \gls*{ir} during compilation;
    \item \emph{graph-based features} that provide information about data and control dependencies during compilation;
    \item \emph{dynamic features} that describe operational aspects in architecture-dependent or architecture-independent ways.
\end{itemize}
%Programming language source code features are language-dependent and dynamic features are expensive to obtain. Our methodology is based on \gls{ir}-level source code and graph-based features as well as it supports estimation of dynamic features.


%\subsection{Obtaining Performance Characteristics}

%\begin{itemize}
%    \item execution time and energy consumption are dynamic features part of the optimization objective;
%    \item they are time-expensive to determine as they require a direct execution of the compiled program;
%    \item the set of features used as input can be rescaled and filtered, to improve the performance of the model itself;
%\end{itemize}

Architecture-dependent dynamic features such as execution time and energy consumption are objectives for compiler optimization, while static features describe programs during compilation~\cite{Allen1970,Schneck1973,Ferrante1984}.
Dynamic features are time-expensive to determine because they require direct execution of compiled programs. This problem can be circumvented through model-based prediction.
The performance of \gls*{ml} models is improved by scaling and filtering the input features~\cite{ashouriSurveyCompilerAutotuning2018,Wang2018}, an example of which is \gls*{pca}~\cite{Härdle2015,Minka2000}.



%\subsection{Selection and Ordering of Optimization Phases}

%\begin{itemize}
%    \item An optimization phase (a.k.a. pass) is a transformation that changes the program with the aim of improving some of its operational characteristics but without changing its functionality.
%    \item A phase may do changes that are not beneficial for a given objective.
%    \item Complex interplay among phases: a phase may enable or disable other phases.
%    \item Proper selection and ordering of phases is instrumental for meeting optimization objectives.
%    \item Optimizing for a single characteristic is typical but resource-constrained systems rather need Pareto optimization of binary size, execution time, and energy consumption.
%    \item Handcrafted sequences and heuristics are not generic and hard to adapt.
%    \item Adaptive and \gls{ml}-based approaches allow adaptation for different scenarios but still has limitations...
%    \item We use an \gls{rl}-based phase selection policy to iteratively predict a phase sequence.
%\end{itemize}

%An optimization phase, also called optimization pass, is a transformation that changes the compiled program for improving some of its operational characteristics but without changing its functionality.
%A phase does changes that are not necessarily  beneficial. For example, reducing code size at the cost of execution time is not appropriate when optimizing for the latter.
%Furthermore, there is a complex interplay among phases: a phase may enable or disable other ones.
%Utility of a phase depends on the current state of the program, the target platform, and the objectives.
%Proper selection and ordering of phases is instrumental for meeting optimization objectives.
%
%Optimizing for a single characteristic, typically execution time or binary size, constitutes a well-studied area. Multi-objective optimization of programs is less researched, while Pareto-optimization of binary size, execution time, and energy consumption suits resource-constrained systems the best.
%
%There are handcrafted phase sequences and heuristics for specific platforms and applications. They are neither generic nor adaptable.
%Adaptive and \gls{ml}-based approaches allow adaptation for different scenarios. Still, they are limited by considering one objective and depending on time-consuming case-by-case profiling.
%We propose an adaptive, \gls{rl}-based phase selection policy that targets multiple relevant objectives with fast \gls{ml}-based estimation of dynamic features.



==> COGUTS - DATE2021 (Copy)3/sections/3_methodology.tex <==
% \begin{figure}[hbtp]
% \centering
% \includesvg[width=.7\linewidth]{images/system_structure.svg}
% \caption{Abstract overview of the conducted research}
% \label{fig:system_structure}
% \end{figure}
\begin{figure*}[t]
    \centering
    \includesvg[width=\linewidth]{images/methodology_v3.svg}
    \caption{The \textit{MLComp} methodology trains and utilizes \acrlong*{pe} and \acrlong*{pss} in four steps.}
    \label{fig:methodology}
    \vspace*{-5mm}
\end{figure*}

%\begin{itemize}
%    \item concept is based on two main components, performance estimator and phase sequence selector
%    \item performance estimator is a fast and efficient way of estimating dynamic features for a given application domain, represented by a set of \emph{target applications}, and a given \emph{target platform}
%    \item it allows accurate prediction adapted for the given domain faster than standard estimation methods
%    \item \emph{phase sequence selector} consists of a policy for combined phase selection and ordering
%    \item the reinforcement learning policy can be adapted for different \emph{target applications} and \emph{target platforms}
%    \item it helps reduce development cost and realize faster time to market by relieving performance engineering from the details of phase selection and ordering
%\end{itemize}

The flow of our methodology is depicted in Fig.~\ref{fig:methodology} and discussed hereafter.
The concept is based on two models:
\begin{enumerate}[leftmargin=*]
    \item \textit{\gls*{pe}} is a fast and efficient way of estimating dynamic features for a given application domain, which is represented by a set of \emph{target applications}, and for a given \emph{target platform}. It allows for accurate prediction adapted to the given domain faster than standard estimation methods.
    \item \textit{\gls*{pss}} is based on a policy for selection and ordering of optimization phases, and supports \gls*{rl}-based adaptation for different \emph{target applications} and \emph{target platforms}. Deploying \gls*{pss} reduces development cost and realizes faster time-to-market by relieving performance engineering from the details of phase selection and ordering.
\end{enumerate}

\subsection{Data Extraction}

%\begin{itemize}
%    \item It refers to box \circled{1} in Fig. \ref{fig:methodology}
%    \item we explore different permutations of optimization phases
%    \item for each permutation we compile the corresponding optimized code and extract the main features.
%    \item the features are extracted from the intermediate representation, therefore this method is independent from programming language and target platform
%    \item the objectives such as execution time, energy consumption and code size are obtained via profiling the compiled code
%    \item the set of all features for all the permutations becomes the training dataset for the performance estimator model
%\end{itemize}

\emph{Data Extraction} is the first step of the methodology. We collect a training dataset for the \gls*{pe} model using the flow depicted in box~\circled{1} in Fig.~\ref{fig:methodology}.
Data is extracted for a target platform from a set of target applications by exploring different permutations of optimization phases. Permutations increase the number of data points as differently optimized variants of programs.
For each combination of permutations and applications, the corresponding optimized code is compiled and its features are collected.
We extract \gls*{ir} features that are similar to those of Milepost GCC \cite{Fursin2011}, such as \gls*{ir} instruction counts, data and control dependencies, loop hierarchies, and call chains. Our tool also extracts platform-specific instruction counts from generated code for \gls*{pe} training.
Dynamic features such as execution time, energy consumption, and code size are obtained via profiling the compiled code.
All features are collected in a dataset that is used  for training the \gls*{pe} model. The size of the dataset depends on the specific set of optimizations and the target applications.

\subsection{Performance Estimator (PE)}

\begin{figure}[h]
\vspace*{-6mm}
\begin{algorithm}[H]
\begin{footnotesize}
\captionsetup{font=footnotesize}
\caption{Model search for fitting the \acrlong*{pe} model}
\label{alg:pe_model_search}
\begin{algorithmic}[1]
\vspace*{-2mm}
\Procedure{ModelSearch}{$input$, $accuracy_{thr}$, $list_{models}$}
\LineComment{We initialize $accuracy_{best}$ to the worst case value, which is $-\infty$}
\LineComment{Higher $accuracy$ is better}
\LineComment{$model_{best}$ is initialized to a dummy one, returning a random value}
\State init $accuracy_{best}$, $model_{best}$
\LineComment{split $input$ into $training$ and $testing$ data}
\State $training$, $testing$ $\gets$ split($input$)
\LineComment{We cycle through all the models}
\For{$model$ in $list_{models}$} \label{alg:pe_model_search_for_loop}
\LineComment{After training the $model$, we test it and check its accuracy}
    \State train($model$, $training$)
    \State $accuracy$ $\gets$ test($model$, $testing$)
    \If{$accuracy$ $>$ $accuracy_{best}$}
        \State $accuracy_{best}$ $\gets$ $accuracy$
        \State $model_{best}$ $\gets$ $model$
    \EndIf
    \If{$accuracy_{best}$ $>$ $accuracy_{thr}$}
        \State \textbf{break for loop}
    \EndIf
\EndFor
\State \textbf{return} $model_{best}$, $accuracy_{best}$
\EndProcedure
\vspace*{0mm}
\end{algorithmic}
\end{footnotesize}
\end{algorithm}
\vspace*{-6mm}
\end{figure}

%\begin{itemize}
%    \item Box \circled{2} in Fig. \ref{fig:methodology}. The performance estimator is used to estimate different characteristics starting from a given set of features
%    \item given a training dataset obtained from a specific set of target applications and corresponding target platform, the training selects the best preprocessing method and best Machine Learning model
%\end{itemize}

The next step is the \emph{\acrlong*{pe} Model Training} in box~\circled{2} in Fig.~\ref{fig:methodology}.
We search for the preprocessing method and \gls*{ml} model that fits the best to the profiling data based on the code features. The list of methods and models to search is given as input. The search process is detailed in Alg.~\ref{alg:pe_model_search}.
Tables~\ref{tab:pe_preprocessing} and~\ref{tab:pe_models} present the preprocessing methods and \gls*{ml} models used by our \gls*{pe} modeling in this paper.
The set of output metrics is completely customizable.
As a training dataset is collected for one target platform, the \gls*{pe} model is to be trained for each target platform separately to achieve high accuracy.
The trained \gls*{pe} model is used in later steps to predict a program's dynamic features from its \gls*{ir} features.


\subsection{Phase Selection Policy}

\begin{figure}[h]
\vspace*{-5mm}
\begin{algorithm}[H]
\begin{footnotesize}
\captionsetup{font=footnotesize}
\caption{Training the Phase Selection Policy}
\label{alg:pss_training}
\begin{algorithmic}[1]
\vspace*{-2mm}
\Procedure{TrainPolicy}{$programs$, $num\_episodes$, $batch\_size$, $learning\_rate$}
\LineComment{Initialize $policy$ to a random one}
\State init $policy$
\LineComment{Perform training episodes in batches}
\State $episode\_count$ $\gets$ $0$
\While{$episode\_count < num\_episodes$}
    \LineComment{Run episodes and then update $policy$}
    \State $list_{episodes}$ $\gets$ init($batch\_size$, $programs$)
    \State $list_{results}$ $\gets$ run($list_{episodes}$, $policy$)
    \State $policy$ $\gets$ optimize($policy$, $learning\_rate$, $list_{results}$)
    \State $episode\_count$ $\gets$ $episode\_count + batch\_size$
\EndWhile
\State \textbf{return} $policy$
\EndProcedure
\vspace*{0mm}
\end{algorithmic}
\end{footnotesize}
\end{algorithm}
\vspace*{-7mm}
\end{figure}


%\begin{itemize}
%    \item It refers to box \circled{3} in Fig. \ref{fig:methodology}
%    \item Phase Selection Policy: tell next best phase to apply
%    \item PE improves training speed by providing quick but accurate estimation of dynamic features.
%    \item Policy is to be trained for new platform (i.e., new PE model) and for new application domain
%\end{itemize}

The trained \gls*{pe} model is used for the \emph{Phase Selection Policy Training} in box~\circled{3} in Fig.~\ref{fig:methodology}.
We use \gls*{rl} to train the policy that selects the best optimization phase to apply to a program characterized by its \gls*{ir} features, and thereby enables an efficient phase sequence to be created iteratively.
The training is done in batches of episodes as listed in Alg.~\ref{alg:pss_training}. The policy is optimized using the REINFORCE \emph{policy gradient method}~\cite{Williams1992,Sutton1999}. The training algorithm creates a phase sequence for a randomly selected target application in each episode with the current policy as depicted in box~\circled{3} in Fig.~\ref{fig:methodology}. The reward in each iteration of an episode reflects how well the last phase changed the dynamic features. Furthermore, the reward guides the training to Pareto-optimal outcomes by penalizing any degradation of the dynamic features. Accumulating rewards over an episode gives a discounted reward, which indicates the overall fitness of the policy for creating a Pareto-optimal phase sequence with respect to final dynamic features. At the end of each batch, the policy is updated according to the episodes' discounted rewards and corresponding phase sequences.
The policy is trained with a given \gls*{pe} and a set of programs that represent a target platform and an application domain, respectively.
The training time is reduced compared to other methods by using \gls*{pe} for fast estimation of dynamic features.
Phase Selection Policy is the model used in the \gls*{pss}.


\subsection{Phase Sequence Selection (PSS)}

%\begin{itemize}
%    \item It refers to box \circled{4} in Fig. \ref{fig:methodology}
%    \item Deploying Phase Selection Policy for selecting phase sequence. Note that PE is not needed for deployment as platform-specific knowledge is incorporated in the trained policy.
%\end{itemize}

The last step of \textit{MLComp} is \emph{Deployment} in box~\circled{4} in Fig.~\ref{fig:methodology}, which is the \gls*{pss} utilizing a trained Phase Selection Policy.
We apply the \gls*{pss} model to drive a compiler's optimizer by selecting phases one after the other.
The policy predicts how probable it is that a phase improves dynamic features of the program and accordingly the phase with the highest probability is applied.
In case the selected phase did not change the program, which might happen because of the uncertainty of the selection, the best predicted phase remains the same for the next iteration. \gls*{pss} overcomes that situation by applying the second best, the third best, and so on until a predefined limit, which is ``Max. inactive subsequence length'' in Table~\ref{tab:pss_training_parameters}.
Phase selection ends when that limit is reached or when the total number of applied phases reaches a threshold.

Note, \gls*{pss} does not require a \gls*{pe} model because the policy learns the platform-specific knowledge.
Decoupling the \gls*{pe} and \gls*{pss} models allows their separate training so that a platform vendor might provide a trained \gls*{pe} model for application developers, who can train a custom \gls*{pss} model with a set of representative applications.

Although the \gls*{pss} model is trained to reach the Pareto-front by selecting locally optimal phases, we observe that both the \gls*{pe} and \gls*{pss} models have \emph{approximation uncertainties} and true Pareto-optimality can not be guaranteed.
The accuracy of \gls*{pss} might be quantified by applying \emph{probabilistic dominance}~\cite{Khosravi2019}, which requires an in-depth empirical evaluation and statistical analysis beyond the scope of this paper. Our evaluation in Section~\ref{sec:evaluation} still shows quasi-Pareto-optimality of the results.


==> COGUTS - DATE2021 (Copy)3/sections/4_experimental_setup.tex <==
\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/experimental_setup.svg}
    \vspace*{-1mm}
    \caption{Detailed toolflow for \textit{MLComp} experimental setup. The process is repeated for each pair of target platform and applications, and it can be adapted for other pairs with minimal code changes.}
    \label{fig:experimental_setup}
\end{figure}

\begin{table}[]
%\resizebox{\linewidth}{!}{%
\footnotesize
\centering
\caption{Preprocessing algorithms evaluated during \gls*{pe} training. The list can easily be expanded, as our framework is customizable with different libraries.}
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{Preprocessing Algorithms}}                \\ \hline
PCA              & Kernel PCA        & NCA                  \\ \hline
Mean-Std Scaling & Min-Max Scaling   & Max-Abs Scaling      \\ \hline
Robust Scaling   & Power Transformer & Quantile Transformer \\ \hline
\end{tabular}%
%}
\label{tab:pe_preprocessing}
\vspace*{-3mm}
\end{table}



\begin{table}[]
%\resizebox{\linewidth}{!}{%
\footnotesize
\centering
\caption{\gls*{ml} models evaluated during \gls*{pe} training. The list can easily be expanded, as our framework is customizable with different libraries.}
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{Machine Learning Regression Models}}                                       \\ \hline
Ridge                     & Kernel Ridge                 & Bayesian Ridge                   \\ \hline
Linear         & SGD               & Passive-Aggressive    \\ \hline
ARD            & Huber             & Theil-Sen             \\ \hline
LARS                      & Lasso                        & Lasso-LARS                       \\ \hline
Support Vector & Nu-Support Vector & Linear Support Vector \\ \hline
ElasticNet                & Orthogonal Matching Pursuit   & Multi-Layer Perceptron           \\ \hline
Decision Tree             & Extra Tree        & Random Forest                    \\ \hline
\end{tabular}
%}
\label{tab:pe_models}
\vspace*{-2mm}
\end{table}

\begin{table}[]
\vspace*{-4mm}
%\footnotesize
%\centering
\caption{Parameters of \gls*{pss} training.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|r|l|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Parameter}} & \multicolumn{1}{|c|}{\textbf{Value}} & \multicolumn{1}{|c|}{\textbf{Parameter}} & \multicolumn{1}{|c|}{\textbf{Value}} \\ \hline
Number of layers & $3$ & Size of inner layer & $16$ \\ \hline
Number of episodes & $512$ & Batch size & $6$ \\ \hline
Max. phase sequence length & $128$ & Learning Rate & $0.1$  \\ \hline
Max. inactive subsequence length & $8$ & & \\ \hline
\end{tabular}%
}
\label{tab:pss_training_parameters}
\vspace*{-2mm}
\end{table}

\begin{table}[]
%\resizebox{\linewidth}{!}{%
\footnotesize
\centering
\caption{LLVM optimization phases used for \gls*{pss} evaluation. The list can easily be expanded. These phases are from optimization levels \texttt{-O3} and \texttt{-Oz}.}
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{Optimization Phases}} \\ \hline
adce & aggressive-instcombine & alignment-from-assumptions \\ \hline
argpromotion & bdce & called-value-propagation \\ \hline
callsite-splitting & constmerge & correlated-propagation \\ \hline
deadargelim & div-rem-pairs & dse \\ \hline
early-cse & early-cse-memssa & elim-avail-extern \\ \hline
float2int & globaldce & globalopt \\ \hline
globals-aa & gvn & indvars \\ \hline
inline & instcombine & instsimplify \\ \hline
ipsccp & jump-threading & licm \\ \hline
loop-deletion & loop-distribute & loop-idiom \\ \hline
loop-load-elim & loop-rotate & loop-sink \\ \hline
loop-unroll & loop-unswitch & loop-vectorize \\ \hline
lower-expect & mem2reg & memcpyopt \\ \hline
mldst-motion & prune-eh & reassociate \\ \hline
sccp & simplifycfg & slp-vectorizer \\ \hline
speculative-execution & sroa & tailcallelim \\ \hline
\end{tabular}%
%}
\label{tab:pss_phases}
\vspace*{-4mm}
\end{table}


%\begin{itemize}
%    %\item custom LLVM build to include the feature extractor and the libraries for running the custom optimization passes
%    \item RAPL\cite{davidRAPLMemoryPower2010} interface for x86 target, to measure used power by processor
%    \item Optuna\cite{optuna_2019}, scikit-learn\cite{scikit-learn} and pandas\cite{rebackPandasdevPandasPandas2020} for training the performance estimator (with FIGURE detailing the flow)
%    \item PyTorch\cite{paszkePyTorchImperativeStyle2019} for training, TorchScript for storing, and LibTorch for deploying the phase sequence selector in LLVM\cite{Lattner2004} (with FIGURE detailing the flow and the single components)
%    \item table containing the parameters used for training the phase sequence selector, further info in text:
%    \begin{itemize}
%        \item 63 code features used as input
%        \item preprocessing method is \gls{pca} with \gls{mle}~\cite{Minka2000}
%    \end{itemize}
%\end{itemize}

%We performed experiments, whose results are reported in Section~\ref{sec:evaluation}, using the following systems and tools.
A detailed toolflow for our experimental setup is shown in Fig. \ref{fig:experimental_setup}. We worked with two different target platforms: profiling for an \emph{x86 target} is done on an Intel Core i7 system using the RAPL~\cite{davidRAPLMemoryPower2010} interface to measure power consumption, and dynamic features for a \emph{RISC-V target} are obtained by accurate simulation with the industrial-grade simulator HIPERSIM~\cite{hipersim} integrated with the open-source McPAT~\cite{Sheng2009}.
Programs are compiled with LLVM~\cite{Lattner2004} version 9.0.0, which is able to target both platforms. The size of the collected dataset depends on the target applications and the set of optimization phases chosen at compile time: in this evaluation, we used between 200 and 600 data points for both the PARSEC benchmark \cite{Bienia2008} on \textit{x86 target} and the BEEBS benchmark \cite{Pallister2013} on \textit{RISC-V target}.

The training of the \gls*{pe} model is implemented in Python using Optuna~\cite{optuna_2019}, scikit-learn~\cite{scikit-learn}, and pandas~\cite{rebackPandasdevPandasPandas2020}. It covers preprocessing methods and \gls*{ml} models listed in Tables~\ref{tab:pe_preprocessing} and~\ref{tab:pe_models}, respectively. The set of output metrics has been chosen to analyze different patterns and distributions. Even though power consumption has a slight correlation with execution time, as in the number of cycles and the number of instructions~\cite{Pallister2015}, increasing the complexity of the system reduces the correlation of these metrics. Therefore, each of them is important for learning the dynamic behaviour of the system.

\gls*{pss} training is implemented also in Python using PyTorch~\cite{paszkePyTorchImperativeStyle2019} for realizing the model. The 63 code features that our static analysis obtains are preprocessed by \gls*{pca} with \gls*{mle}~\cite{Minka2000} before being passed to Deep \gls*{rl}~\cite{Francois-lavet2018}. The \gls*{pss} model is trained with the parameters listed in Table~\ref{tab:pss_training_parameters}, applying optimization phases shown in Table~\ref{tab:pss_phases}.
The trained model is stored in TorchScript format, to be loaded into and utilized by our custom LLVM optimization with LibTorch, the PyTorch C++ API.

Note that \gls*{pe} and \gls*{pss} are independent of the target platform and the used application set. The necessary adaptations when changing the target platform are limited to adjusting target-specific compiler flags and utilizing a tool with support for gathering dynamic features inside the \emph{Data Extraction} block. Furthermore, any application can be used with our training frameworks as long as it supports a build method using LLVM and allows controlling optimization phases via parameters or environment variables.

==> COGUTS - DATE2021 (Copy)3/sections/5_evaluation.tex <==
To evaluate our \textit{MLComp} methodology, we trained and tested both \gls*{pe} and \gls*{pss} models on different target platforms with different benchmarks as target applications.


\subsection{PARSEC Benchmark Evaluation on x86 Platform}

\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/results/pe_x86_parsec_paper_v4.svg}
    \caption{Comparison between profiling data and prediction of a trained \gls*{pe} model for PARSEC benchmark applications on x86 platform shows very similar distributions, which supports the efficacy and accuracy of our model.}
    \label{fig:pe_x86_parsec}
    \vspace*{-3mm}
\end{figure}

Here we focus our analysis on the PARSEC benchmark \cite{Bienia2008}, running on an x86 platform. First, we gather the required dataset by profiling the execution of programs from the benchmark compiled with different optimization phases. Then, we use our framework to train different \gls*{ml} models and select the best one; the results are shown in Fig. \ref{fig:pe_x86_parsec}. As we can see, the exact distributions and the ones generated by our \gls*{pe} model are almost identical for all the 4 metrics.
Note that the \textit{blackscholes} benchmark has a very tight distribution, while all the others have wider distributions. Referring to \circled{1}, we can see that the only visible difference resides in the \textit{facesim} benchmark. However, there is always a high fidelity, as the error between the correct and the predicted distributions always has the same bias. This property is important for the training of the \gls*{pss} model, giving the correct positive/negative reward to the current choice, even if a limited prediction error is present.

\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/results/pss_x86_parsec_1_paper_v5.svg}
    \caption{\gls*{pss} validation results for PARSEC applications on x86 platform. Values are relative to those of unoptimized code, the lower is the better.}
    \label{fig:pss_x86_parsec}
    \vspace*{-2mm}
\end{figure}

After validating the \gls*{pe} model, we used it to train the corresponding \gls*{pss} model. In Fig. \ref{fig:pss_x86_parsec}, we can see the result of the validation executed after the training. Specifically, distributions are pretty similar across standard state-of-the-art optimizations and \textit{MLComp}. However, in some cases, as shown by \circled{1} and \circled{3}, some standard phase usage can increase both the energy consumption and the execution time between 8x and 10x, respectively, while \textit{MLComp} shows slight improvements. Regarding memory size, as pointed by \circled{2}, there are minimal gains, which could be related to the benchmarks being synthetic applications.

\subsection{BEEBS Benchmark Evaluation on RISC-V Platform}

\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/results/pe_riscv_beebs_paper_v3.svg}
    \caption{Comparison between profiling data and prediction of a trained \gls*{pe} model for BEEBS benchmark applications on RISC-V platform.}
    \label{fig:pe_riscv_beebs}
    \vspace*{-3mm}
\end{figure}

We performed a similar evaluation for BEEBS \cite{Pallister2013} on the RISC-V platform. In this case, the number of benchmarks is much higher compared to PARSEC, and since the \gls*{pe} results are similar to those with PARSEC, we show only an overview of the distribution points in Fig. \ref{fig:pe_riscv_beebs}.

\begin{figure}[t]
    \centering
    \includesvg[width=\linewidth]{images/results/pss_riscv_beebs_2_paper_v5.svg}
    \caption{\gls*{pss} validation results for BEEBS applications on RISC-V platform. Values are relative to those of unoptimized code, the lower is the better.}
    \label{fig:pss_riscv_beebs}
    \vspace*{-4mm}
\end{figure}

This \gls*{pe} model was then used to train a \gls*{pss} model, obtaining the results shown in Fig. \ref{fig:pss_riscv_beebs}. Here, at pointer \circled{1}, we can see that our \textit{MLComp} performs better on average than standard state-of-the-art policies: reducing energy while also optimizing other objectives. Also with BEEBS, we can see that the memory size does not improve or worsen much, as pointed by \circled{2}. In addition, \textit{MLComp} results in similar patterns of execution time and energy consumption. Focusing on pointer \circled{3}, we can see how our \textit{MLComp} obtain more balanced results compared to standard state-of-the-art policies.

\subsection{Discussion and Key Takeaways}

Our \gls*{pe} model has a maximum percentage error \textit{smaller than 2\%} across all four metrics, while that of the comparable state of the art is in the range of 2\%-7\% on a single metric \cite{diopPowerModelingHeterogeneous2014, balaprakashAutoMOMMLAutomaticMultiobjective2016,liAccurateEfficientProcessor2009,bonaEnergyEstimationOptimization2002,vandensteenAnalyticalProcessorPerformance2016,laurentFunctionalLevelPower2004}.
Moreover, the efficient setup for data extraction and the heuristic search of models help us to reach higher accuracy with less time spent for acquiring data and training the model. Profiling the applications and training the models took \textit{only 2 days}, compared to 15, 30 or 108 days \cite{laurentFunctionalLevelPower2004, bonaEnergyEstimationOptimization2002}.
%while requiring more time to acquire the data and train the model. This is related to the more efficient setup for data extraction, as well as the heuristic search which is capable of comparing different models to train the most accurate one.

Drawing a straight comparison is more difficult for our \gls*{pss} model, as related techniques optimize a single objective only.
The state-of-the-art results oscillate between 5\% and 30\% improvement in execution time~\cite{Ashouri2017,Ashouri2016a}, which makes our results fall in their average with up to 12\% improvement in that metric.
However, our \gls*{pss} model considers additional objectives and reaches up to 6\% reduction in energy consumption while not increasing code size. There is actually a slight 0.1\% improvement in the latter.
%Looking at our \gls{pss} model, it is more difficult to draw a line of comparison with state of the art, as they focus on obtaining the best result on a single objective for a given application. These works oscillate between 5\% and 30\% regarding execution time. Therefore, with an improvement of up to 12\%, our \textit{MLComp} methodology falls in the average of these improvements.
%However, other works do not consider multiple objectives, for which we provide up to 6\% reduction in energy consumption and further improvements in code size, around 0.1\%, mostly in terms of code cluttering.
%Moreover, compilation time is longer due to the dynamic profiling, while with \textit{MLComp} the overhead is present only at training time, and therefore compilation is comparable with standard optimization algorithms.


We can summarize the following key observations:

\begin{itemize}[leftmargin=*]
    \item The \gls*{pe} model realizes fast estimation with high accuracy, as it is capable of reproducing the profiled distributions.
    \item The \gls*{pss} model performs better than standard optimizations on average and also provides quasi-optimal results for multiple objectives.
    \item Our \textit{MLComp} methodology is fully automated and is usable with different target platforms and applications, enabling for fast estimation and optimization without manual analysis and modeling required.
\end{itemize}

% \begin{figure}[hbtp]
% \centering
% \includegraphics[width=\linewidth]{images/results/parsec_pe.pdf}
% %\vspace*{-4mm}
% \caption{PARSEC estimation using trained Performance Estimator.}%: many solutions have the same or very close indicator results, so they are overlapped. Efficiency could be improved upon but this is also related to the older technology library than current state-of-the-art.}
% \label{fig:parsec_pe}
% %\vspace*{-1mm}
% \end{figure}

% \begin{itemize}
%     \item In Fig. \ref{fig:parsec_pe} we can see a comparison of the objecties obtained via profiling of PARSEC benchmarks on x86 platform and the estimation of our Machine Learning model
%     \item their distributions are very similar, with the maximum percentage absolute error being less than 10\%
%     \item our estimator model can then be used to accurately estimate these objectives while training the phase selection policy
%     \item most importantly it has very high fidelity, that is if A $>$ B using the correct simulation, the relation holds also for our model
% \end{itemize}

% \begin{figure}[hbtp]
% \centering
% \includegraphics[width=\linewidth]{images/results/riscv_beebs_2.pdf}
% %\vspace*{-4mm}
% \caption{RISC-V BEEBS optimization goals compared to unoptimized code.}%: many solutions have the same or very close indicator results, so they are overlapped. Efficiency could be improved upon but this is also related to the older technology library than current state-of-the-art.}
% \label{fig:riscv_beebs_pss}
% %\vspace*{-1mm}
% \end{figure}

% \begin{itemize}
%     \item In Fig. \ref{fig:riscv_beebs_pss} we can see the results for different objectives on the RISCV BEEBS benchmark.
%     \item The distributions are similar, overall our Phase Selection Policy tends to improve the average case by a few percentage points compared to other standard optimization algorithms.
%     \item these improvements cover at the same time different objectives, therefore our methodology is capable of reaching Pareto-optimal points in multiobjective optimization
% \end{itemize}

% \begin{itemize}
%     \item Analysis and comparison of accuracy of different platforms and applications for the performance estimator
%     \item comparison with other state-of-the-art works covering PARSEC/RISC-V BEEBS
%     \item analysis of phase sequence selector against standard -O3 and -Oz, both for RISC-V and PARSEC. On RISC-V the gains are limited, which may be related to the lower complexity of the benchmarks and of the platform compared to x86/PARSEC
% \end{itemize}

==> COGUTS - DATE2021 (Copy)3/sections/6_related.tex <==

\subsection{Performance Modeling}

%\begin{itemize}
%    \item \cite{balaprakashAutoMOMMLAutomaticMultiobjective2016} uses different preprocessing techniques to enhance the data before training a ML algorithm. The selection of ML models is limited to simple ones, such as linear regression and regression forests; data extraction is executed using RAPL, thus at component-level; it focuses only on power estimation, although covering different components (processor, memory);
%    \item \cite{diopPowerModelingHeterogeneous2014} employs both functional modeling and ML modeling, however there is only a linear regression model being tested; data extraction still uses hardware registers, but at a lower-level compared to RAPL; it focuses only on power, neglecting execution time;
%    \item \cite{liAccurateEfficientProcessor2009} employs regression trees to estimate power, using a simulator to increase the number of samples and thus the accuracy, thus providing a trade-off between training length and accuracy;
%\end{itemize}

The work presented in~\cite{balaprakashAutoMOMMLAutomaticMultiobjective2016} performs \gls*{ml}-based power estimation. The training is based on component-level data that is extracted using RAPL and enhanced by different preprocessing techniques. The selection of considered \gls*{ml} models is limited to simple ones, such as linear regression and regression forests.
A different approach for power estimation is described in~\cite{diopPowerModelingHeterogeneous2014}, which employs both functional and \gls{ml} modeling. A linear regression model is tested with training data, which is extracted from hardware registers but at a lower-level than RAPL.
The technique in~\cite{liAccurateEfficientProcessor2009} estimates power using regression trees. The authors use a simulator to increase the number of samples and thus improve accuracy. The described method allows trading off training time for estimation accuracy.

\subsection{Compiler Optimizations}

%\begin{itemize}
%    \item ML-based approaches for optimization phases: \cite{Wang2018}; and for phase selection and ordering: \cite{ashouriSurveyCompilerAutotuning2018}
%    \item \gls{sl} approaches COBAYN \cite{Ashouri2014,Ashouri2016} and Milepost GCC \cite{Fursin2011} do phase selection for execution time and the latter also for code size. They do not consider phase ordering.
%    \item However, it has been shown that order of phases is important for energy consumption \cite{Pallister2015}. They also show that the structure of a benchmark has large effect on the effectiveness of optimizations.
%    \item \cite{Blackmore2017} uses iterative compilation to adapt a static phase order for a set of benchmarks with respect to execution time objective.
%    \item MiCOMP \cite{Ashouri2017} is a \gls{sl} approach for phase ordering with respect to execution time objective. Profiling is used not only for training but also in deployment before optimizing a program.
%    \item MiCOMP predicts a whole sequence at once, no other recent work does that for phase ordering. Constructing a phase sequence iteratively by selecting the next best phase step by step is an easier learning problem and allows more flexibility. Major recent works, like the followings, take that approach.
%    \item \cite{Kulkarni2012} is an \gls{rl}-based approach for phase ordering with execution time objective. It is implemented for Java JIT in Jikes RVM.
%    \item \cite{Ashouri2016a} does \gls{sl} for phase ordering with execution time objective.
%    \item All approaches are trained on data collected from actual execution.
%\end{itemize}

\gls*{ml}-based approaches are used in compiler optimizations in general~\cite{Wang2018} and for phase selection and ordering in particular~\cite{ashouriSurveyCompilerAutotuning2018}.
The properties of major related works discussed here are also summarized in Table~\ref{tab:pss}.
COBAYN \cite{Ashouri2016,Ashouri2014} and Milepost GCC \cite{Fursin2011} are \gls*{sl} approaches optimizing for execution time, and also for code size in the latter case. They handle phase selection but ignore the order of phases, which affects the quality of generated code~\cite{Pallister2015}.
The iterative compilation approach in~\cite{Blackmore2017} adapts a static phase order for a set of benchmarks and optimizes execution time.
MiCOMP~\cite{Ashouri2017} uses \gls*{sl} to train a model that predicts complete phase sequences optimized for execution time. %MiCOMP uses profiling-based dynamic features of unoptimized programs as input for the phase sequence prediction.

Predicting a phase sequence at once, like MiCOMP does, is challenging because of the high complexity of the action space. Constructing a phase sequence iteratively is an easier learning problem and allows more flexibility. Major recent works as well as our methodology follow the iterative approach.
An \gls*{rl}-based technique is reported in~\cite{Kulkarni2012} for creating a phase sequence in a Java JIT compiler optimizing execution time.
An iterative phase sequence prediction methodology is described in~\cite{Ashouri2016a}, which is based on \gls*{sl} and also optimizes execution time.
It is noteworthy that all these approaches train models on data collected from actual execution.


==> COGUTS - DATE2021 (Copy)3/sections/7_conclusion.tex <==
%\begin{itemize}
%    \item Software running on resource-constrained embedded systems for \gls{iot} and \gls{cps} applications need to be extremely optimized for specific hardware.
%    \item Many standard optimization phases are available in major optimizing compilers but proper selection and ordering of phases to apply for a given system is a complex problem. The state of the art has limitations.
%    \item We proposed an \gls{rl}-based phase selection policy that allows adaptive selection of Pareto-optimal optimization sequences.
%    \item We also proposed an \gls{ml}-based performance estimator that encapsulates relevant knowledge about the platform to speed up training of the phase selection policy.
%    \item We implemented training frameworks for the proposed models and integrated phase sequence selector into LLVM
%    \item Our evaluation shows that...
%\end{itemize}

%Embedded systems for \gls{iot} and \gls{cps} applications operate on limited time, power and memory budgets, and so their software is subjected to extreme platform-dependent optimization requirements.
%While many powerful optimization phases are available in major optimizing compilers, proper selection and ordering of them still requires expert knowledge because of their target- and inter-dependencies. State-of-the-art solutions can be applied case by case but their adaption is expensive and they cover only a limited set of optimization objectives.

We propose the \textit{MLComp} methodology to overcome limitations of current solutions in compiler optimization phase sequencing and performance modeling.
State-of-the-art optimizers can be applied for different target platforms and applications case by case, but their adaptation is expensive and they typically optimize one metric only.
\textit{MLComp} supports adaptive selection of Pareto-optimal phase sequences with respect to execution time, power consumption, and code size by a \acrfull*{pss} with an \gls*{rl}-based policy. Fast adaptation of the policy for different target platforms and application domains is enabled by an \gls*{ml}-based \acrfull*{pe} model, which provides fast-yet-accurate prediction of dynamic program features. The \gls*{pe} model is trained for a target platform by automatically selecting the most suitable data preprocessing method and \gls*{ml} model for accurate prediction. This is a novel contribution in performance modeling as current solutions require manual analysis and modeling.
Experiments with LLVM on the x86 and RISC-V platforms show that our methodology is efficiently reusable with different target platforms and applications. The \gls*{pe} model realizes fast estimation with very high accuracy, and the \gls*{pss} model performs better than state-of-the-art optimizations with multiple objectives.


==> COGUTS - DATE2021 (Copy)3/sections/a1_reviews.tex <==
\clearpage

\appendix

\textbf{DATE 2021 Reviews for Submission 1876}

\textbf{Title:} MLComp: A Methodology for Machine Learning-based Performance Estimation and Adaptive Selection of Pareto-Optimal Compiler Optimization Sequences


\textbf{Authors:} Alessio Colucci, Dávid Juhász, Martin Mosbeck, Alberto Marchisio, Semeen Rehman, Manfred Kreutzer, Guenther Nadbath, Axel Jantsch and Muhammad Shafique


\subsection{REVIEWER 1}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 2

\subsubsection{Summary of ideas}
Optimization phase ordering in compilers is a know and well-studied field. Machine learning approaches have been proposed in the past to devise the best ordering for a particular class of applications and/or a particular architectural target. State-of-the-art solutions suffer from two main shortcomings:
\begin{enumerate}
    \item they optimize for a specific metric at a time, while in embedded systems - the focus of this paper - it is typically desireable to optimize for multiple objective functions (time, energy, code size...);
    \item they require time consuming adaptation to different targets, as they leverage profiling at their core.
\end{enumerate}

This paper addresses these shortcomings: 
\begin{enumerate}
    \item it supports adaptive selection of phases (pareto-optimal with respect to several metrics) based on reinforcement learning;
    \item it enables fast adaptation to different targets/application domains via a ML-based performance estimator, which predicts dynamic program features based on IR-based (static code analysis) ones.
\end{enumerate}

\subsubsection{Strong points}
\begin{itemize}
    \item tackles a relevant and challenging problem
    \item excellent presentation overall
    \item builds on a solid base of methods and tools
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item maybe a bit incremental w.r.t. previous work
\end{itemize}


\subsubsection{Other comments}
\begin{itemize}
    \item In the introduction (starting on the last paragraph before the bullet list) you describe Tables I and II. At this stage you haven't introduced the acronym SL yet, nor the name of your tool (both in the table).
    \item You might want to use more contrasting colors for Figures 4 to 7, such that the key messages are conveyed also when the paper is printed in B/W.
\end{itemize}


\subsection{REVIEWER 2}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
This paper presents a methodology for selecting the pareto-optimal sequence of compiler optimizations. Specifically, authors propose a reinforcement learning based approach. Additionally, a machine-learning based approach is proposed for performance estimation, which, in turn is required for optimization sequencing. The approach is evaluated on x86 platform and RiSC-V based platform and its effectiveness is demonstrated.


\subsubsection{Strong points}
\begin{itemize}
    \item The presentation is good
    \item The targeted problem is well motivated
    \item The experimental results are good and comprehensive
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item The vague idea on optimality
    \item The requirement of training 
    \item PE model seems to be quite straightforward
\end{itemize}

\subsubsection{Other comments}
\begin{itemize}
    \item Overall, this is a nice paper. The problem is well motivated and the solution is mostly well presented. I also like the part where authors took effort in applying the technique for two different target platforms i.e. x86 based platform and a RISC-V based platform. The validation of the proposed technique is comprehensive. 
    \item The usage of reinforcement learning for selecting optimal sequence seems to be a novel application of reinforcement learning. 
    \item On the downside, I found the optimality of the phase sequence selection (PSS) quite questionable. What the approach is targeting is more like a greedy heuristic where the option is chosen that improves the dynamic features with the highest probability and continue to do so with second/third best. However, the probabilities itself are estimates and it is unlikely that such a solution can be optimal. 
    \item As with any machine learning approach, the performance estimation model needs the training data. Also this model seems to be quite naive and totally reliant on the amount of training data available. 
    \item Finally, I would have liked a more in-depth description of the reinforcement learning part. Currently, it is too short for the reader who wish to independently reproduce the results. In contrast, I think that Algorithm 1 (PE model) is quite trivial and can be removed for explaining more important things.
\end{itemize}

\subsection{REVIEWER 3}

\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
The work uses reinforcement learning to control the sequence of compiler optimizations applied. A novel performance estimation is used to reduce the time for dynamic profiling.

\subsubsection{Strong points}
\begin{itemize}
    \item The paper is well-written and targets an important topic.
    \item The related works are quite comprehensive.
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item My main concerns with the paper are in the results and analysis. Figures 4 to 7 do not compare the performance of the code with the recommended optimization sequence from the proposed tool with other frameworks that also search the optimization space for better performance. Instead, the authors primarily compare their performance to the unoptimized code.
    \item The authors should implement the best hand-optimized version of the code and use that as one of the baselines.
\end{itemize}

\subsection{REVIEWER 4}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
Having good models for performance estimation is key when selecting optimization parameters and the order of sequences during compilation. The search space, depending on different target architectures and applications, is incredibly large. Thus, the authors propose a reinforcement learning-based approach, which steers the selection of sequences with respect to execution time, power consumption, and code size adaptively. The method is evaluated for two different processor architectures.

\subsubsection{Strong points}
\begin{itemize}
    \item The paper is structured and well-written
    \item The paper deal with an important topic
    \item ML-based prediction of metrics is very good
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item The training phase is difficult to follow
    \item Taking a lax look at the concept of Pareto optimality
\end{itemize} 

\subsubsection{Other comments}
\begin{itemize}
    \item Since most applications show a high distribution of the considered metrics, Pareto optimality is not given. Here, rather a probabilistic dominance criterion should be considered.
    \item Tables I and II provide a nice comparison with related work. Further, a high prediction accuracy is demonstrated. But, what I miss in the experiments is an overall evaluation in comparison to other approaches (e.g., Milepost).
    \item Abbreviations should be introduced at their first occurrence.
    \item The entire paper should be carefully proofread for grammar and spelling mistakes (see the non-comprehensive list below).
    \item \textbf{Typos and grammar mistakes:}
    \begin{itemize}
        \item in abstract: "methdology" => "methodology"
        \item p. 1: "knowledge on the internal details" => "knowledge of the internal details"
        \item p. 2: "A compiler converts source code into executable" => "A compiler converts source code into an executable"
        \item p. 3: "in Algorihm 2." => "in Algorithm 2."
        \item p. 3: "with respects to" => "with respect to"
        \item p. 4: "The training of the PE model is implemented in Python using Optuna [37], scikit-learn [38], and pandas [39] and covers..." => "The training of the PE model is implemented in Python using Optuna [37], scikit-learn [38], and pandas [39]. It covers..."
        \item p. 5: "the error between the correct and the predicted distributions have always" => "the error between the correct and the predicted distributions always has"
        \item p. 5: "In Fig. 5 we can" => "In Fig. 5, we can"
        \item p. 6: "a ML-based" => "an ML-based"
    \end{itemize}
\end{itemize}

==> sections/6_related.tex <==

\subsection{Performance Modeling}

%\begin{itemize}
%    \item \cite{balaprakashAutoMOMMLAutomaticMultiobjective2016} uses different preprocessing techniques to enhance the data before training a ML algorithm. The selection of ML models is limited to simple ones, such as linear regression and regression forests; data extraction is executed using RAPL, thus at component-level; it focuses only on power estimation, although covering different components (processor, memory);
%    \item \cite{diopPowerModelingHeterogeneous2014} employs both functional modeling and ML modeling, however there is only a linear regression model being tested; data extraction still uses hardware registers, but at a lower-level compared to RAPL; it focuses only on power, neglecting execution time;
%    \item \cite{liAccurateEfficientProcessor2009} employs regression trees to estimate power, using a simulator to increase the number of samples and thus the accuracy, thus providing a trade-off between training length and accuracy;
%\end{itemize}

The work presented in~\cite{balaprakashAutoMOMMLAutomaticMultiobjective2016} performs \gls*{ml}-based power estimation. The training is based on component-level data that is extracted using RAPL and enhanced by different preprocessing techniques. The selection of considered \gls*{ml} models is limited to simple ones, such as linear regression and regression forests.
A different approach for power estimation is described in~\cite{diopPowerModelingHeterogeneous2014}, which employs both functional and \gls{ml} modeling. A linear regression model is tested with training data, which is extracted from hardware registers but at a lower-level than RAPL.
The technique in~\cite{liAccurateEfficientProcessor2009} estimates power using regression trees. The authors use a simulator to increase the number of samples and thus improve accuracy. The described method allows trading off training time for estimation accuracy.

\subsection{Compiler Optimizations}

%\begin{itemize}
%    \item ML-based approaches for optimization phases: \cite{Wang2018}; and for phase selection and ordering: \cite{ashouriSurveyCompilerAutotuning2018}
%    \item \gls{sl} approaches COBAYN \cite{Ashouri2014,Ashouri2016} and Milepost GCC \cite{Fursin2011} do phase selection for execution time and the latter also for code size. They do not consider phase ordering.
%    \item However, it has been shown that order of phases is important for energy consumption \cite{Pallister2015}. They also show that the structure of a benchmark has large effect on the effectiveness of optimizations.
%    \item \cite{Blackmore2017} uses iterative compilation to adapt a static phase order for a set of benchmarks with respect to execution time objective.
%    \item MiCOMP \cite{Ashouri2017} is a \gls{sl} approach for phase ordering with respect to execution time objective. Profiling is used not only for training but also in deployment before optimizing a program.
%    \item MiCOMP predicts a whole sequence at once, no other recent work does that for phase ordering. Constructing a phase sequence iteratively by selecting the next best phase step by step is an easier learning problem and allows more flexibility. Major recent works, like the followings, take that approach.
%    \item \cite{Kulkarni2012} is an \gls{rl}-based approach for phase ordering with execution time objective. It is implemented for Java JIT in Jikes RVM.
%    \item \cite{Ashouri2016a} does \gls{sl} for phase ordering with execution time objective.
%    \item All approaches are trained on data collected from actual execution.
%\end{itemize}

\gls*{ml}-based approaches are used in compiler optimizations in general~\cite{Wang2018} and for phase selection and ordering in particular~\cite{ashouriSurveyCompilerAutotuning2018}.
The properties of major related works discussed here are also summarized in Table~\ref{tab:pss}.
COBAYN \cite{Ashouri2016,Ashouri2014} and Milepost GCC \cite{Fursin2011} are \gls*{sl} approaches optimizing for execution time, and also for code size in the latter case. They handle phase selection but ignore the order of phases, which affects the quality of generated code~\cite{Pallister2015}.
The iterative compilation approach in~\cite{Blackmore2017} adapts a static phase order for a set of benchmarks and optimizes execution time.
MiCOMP~\cite{Ashouri2017} uses \gls*{sl} to train a model that predicts complete phase sequences optimized for execution time. %MiCOMP uses profiling-based dynamic features of unoptimized programs as input for the phase sequence prediction.

Predicting a phase sequence at once, like MiCOMP does, is challenging because of the high complexity of the action space. Constructing a phase sequence iteratively is an easier learning problem and allows more flexibility. Major recent works as well as our methodology follow the iterative approach.
An \gls*{rl}-based technique is reported in~\cite{Kulkarni2012} for creating a phase sequence in a Java JIT compiler optimizing execution time.
An iterative phase sequence prediction methodology is described in~\cite{Ashouri2016a}, which is based on \gls*{sl} and also optimizes execution time.
It is noteworthy that all these approaches train models on data collected from actual execution.


==> sections/a1_reviews.tex <==
\clearpage

\appendix

\textbf{DATE 2021 Reviews for Submission 1876}

\textbf{Title:} MLComp: A Methodology for Machine Learning-based Performance Estimation and Adaptive Selection of Pareto-Optimal Compiler Optimization Sequences


\textbf{Authors:} Alessio Colucci, Dávid Juhász, Martin Mosbeck, Alberto Marchisio, Semeen Rehman, Manfred Kreutzer, Guenther Nadbath, Axel Jantsch and Muhammad Shafique


\subsection{REVIEWER 1}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 2

\subsubsection{Summary of ideas}
Optimization phase ordering in compilers is a know and well-studied field. Machine learning approaches have been proposed in the past to devise the best ordering for a particular class of applications and/or a particular architectural target. State-of-the-art solutions suffer from two main shortcomings:
\begin{enumerate}
    \item they optimize for a specific metric at a time, while in embedded systems - the focus of this paper - it is typically desireable to optimize for multiple objective functions (time, energy, code size...);
    \item they require time consuming adaptation to different targets, as they leverage profiling at their core.
\end{enumerate}

This paper addresses these shortcomings: 
\begin{enumerate}
    \item it supports adaptive selection of phases (pareto-optimal with respect to several metrics) based on reinforcement learning;
    \item it enables fast adaptation to different targets/application domains via a ML-based performance estimator, which predicts dynamic program features based on IR-based (static code analysis) ones.
\end{enumerate}

\subsubsection{Strong points}
\begin{itemize}
    \item tackles a relevant and challenging problem
    \item excellent presentation overall
    \item builds on a solid base of methods and tools
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item maybe a bit incremental w.r.t. previous work
\end{itemize}


\subsubsection{Other comments}
\begin{itemize}
    \item In the introduction (starting on the last paragraph before the bullet list) you describe Tables I and II. At this stage you haven't introduced the acronym SL yet, nor the name of your tool (both in the table).
    \item You might want to use more contrasting colors for Figures 4 to 7, such that the key messages are conveyed also when the paper is printed in B/W.
\end{itemize}


\subsection{REVIEWER 2}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
This paper presents a methodology for selecting the pareto-optimal sequence of compiler optimizations. Specifically, authors propose a reinforcement learning based approach. Additionally, a machine-learning based approach is proposed for performance estimation, which, in turn is required for optimization sequencing. The approach is evaluated on x86 platform and RiSC-V based platform and its effectiveness is demonstrated.


\subsubsection{Strong points}
\begin{itemize}
    \item The presentation is good
    \item The targeted problem is well motivated
    \item The experimental results are good and comprehensive
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item The vague idea on optimality
    \item The requirement of training 
    \item PE model seems to be quite straightforward
\end{itemize}

\subsubsection{Other comments}
\begin{itemize}
    \item Overall, this is a nice paper. The problem is well motivated and the solution is mostly well presented. I also like the part where authors took effort in applying the technique for two different target platforms i.e. x86 based platform and a RISC-V based platform. The validation of the proposed technique is comprehensive. 
    \item The usage of reinforcement learning for selecting optimal sequence seems to be a novel application of reinforcement learning. 
    \item On the downside, I found the optimality of the phase sequence selection (PSS) quite questionable. What the approach is targeting is more like a greedy heuristic where the option is chosen that improves the dynamic features with the highest probability and continue to do so with second/third best. However, the probabilities itself are estimates and it is unlikely that such a solution can be optimal. 
    \item As with any machine learning approach, the performance estimation model needs the training data. Also this model seems to be quite naive and totally reliant on the amount of training data available. 
    \item Finally, I would have liked a more in-depth description of the reinforcement learning part. Currently, it is too short for the reader who wish to independently reproduce the results. In contrast, I think that Algorithm 1 (PE model) is quite trivial and can be removed for explaining more important things.
\end{itemize}

\subsection{REVIEWER 3}

\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
The work uses reinforcement learning to control the sequence of compiler optimizations applied. A novel performance estimation is used to reduce the time for dynamic profiling.

\subsubsection{Strong points}
\begin{itemize}
    \item The paper is well-written and targets an important topic.
    \item The related works are quite comprehensive.
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item My main concerns with the paper are in the results and analysis. Figures 4 to 7 do not compare the performance of the code with the recommended optimization sequence from the proposed tool with other frameworks that also search the optimization space for better performance. Instead, the authors primarily compare their performance to the unoptimized code.
    \item The authors should implement the best hand-optimized version of the code and use that as one of the baselines.
\end{itemize}

\subsection{REVIEWER 4}
\subsubsection{Reviewer's Scores}
\textbf{Overall Value:} 1

\subsubsection{Summary of ideas}
Having good models for performance estimation is key when selecting optimization parameters and the order of sequences during compilation. The search space, depending on different target architectures and applications, is incredibly large. Thus, the authors propose a reinforcement learning-based approach, which steers the selection of sequences with respect to execution time, power consumption, and code size adaptively. The method is evaluated for two different processor architectures.

\subsubsection{Strong points}
\begin{itemize}
    \item The paper is structured and well-written
    \item The paper deal with an important topic
    \item ML-based prediction of metrics is very good
\end{itemize}

\subsubsection{Weak points}
\begin{itemize}
    \item The training phase is difficult to follow
    \item Taking a lax look at the concept of Pareto optimality
\end{itemize} 

\subsubsection{Other comments}
\begin{itemize}
    \item Since most applications show a high distribution of the considered metrics, Pareto optimality is not given. Here, rather a probabilistic dominance criterion should be considered.
    \item Tables I and II provide a nice comparison with related work. Further, a high prediction accuracy is demonstrated. But, what I miss in the experiments is an overall evaluation in comparison to other approaches (e.g., Milepost).
    \item Abbreviations should be introduced at their first occurrence.
    \item The entire paper should be carefully proofread for grammar and spelling mistakes (see the non-comprehensive list below).
    \item \textbf{Typos and grammar mistakes:}
    \begin{itemize}
        \item in abstract: "methdology" => "methodology"
        \item p. 1: "knowledge on the internal details" => "knowledge of the internal details"
        \item p. 2: "A compiler converts source code into executable" => "A compiler converts source code into an executable"
        \item p. 3: "in Algorihm 2." => "in Algorithm 2."
        \item p. 3: "with respects to" => "with respect to"
        \item p. 4: "The training of the PE model is implemented in Python using Optuna [37], scikit-learn [38], and pandas [39] and covers..." => "The training of the PE model is implemented in Python using Optuna [37], scikit-learn [38], and pandas [39]. It covers..."
        \item p. 5: "the error between the correct and the predicted distributions have always" => "the error between the correct and the predicted distributions always has"
        \item p. 5: "In Fig. 5 we can" => "In Fig. 5, we can"
        \item p. 6: "a ML-based" => "an ML-based"
    \end{itemize}
\end{itemize}
